The Tracking Tapered Gridded Estimator for the 21-cm power spectrum from MWA drift scan observations I: Validation and preliminary results

Drift scan observations provide the broad sky coverage and instrumental stability needed to measure the Epoch of Reionization (EoR) 21-cm signal. In such observations, the telescope's pointing center (PC) moves continuously on the sky. The Tracking Tapered Gridded Estimator (TTGE) combines observations from different PC to estimate $P(k_{\perp}, k_{\parallel})$ the 21-cm power spectrum, centered on a tracking center (TC) which remains fixed on the sky. The tapering further restricts the sky response to a small angular region around TC, thereby mitigating wide-field foregrounds. Here we consider $154.2 \, {\rm MHz}$ ($z = 8.2$) Murchison Widefield Array (MWA) drift scan observations. The periodic pattern of flagged channels, present in MWA data, is known to introduce artefacts which pose a challenge for estimating $P(k_{\perp}, k_{\parallel})$. We demonstrate that the TTGE is able to recover $P(k_{\perp}, k_{\parallel})$ without any artefacts, and estimate $P(k)$ within $5 \%$ accuracy over a large $k$-range. We also present preliminary results for a single PC, combining 9 nights of observation $(17 \, {\rm min}$ total). We find that $P(k_{\perp}, k_{\parallel})$ exhibits streaks at a fixed interval of $k_{\parallel}=0.29 \, {\rm Mpc}^{-1}$, which matches $\Delta \nu_{\rm per}=1.28 \, {\rm MHz}$ that is the period of the flagged channels. The streaks are not as pronounced at larger $k_{\parallel}$, and in some cases they do not appear to extend across the entire $k_{\perp}$ range. The rectangular region $0.05 \leq k_{\perp} \leq 0.16 \, {\rm Mpc^{-1}}$ and $0.9 \leq k_{\parallel} \leq 4.6 \, {\rm Mpc^{-1}}$ is found to be relatively free of foreground contamination and artefacts, and we have used this to place the $2\sigma$ upper limit $\Delta^2(k) < (1.85 \times 10^4)^2\, {\rm mK^2}$ on the EoR 21-cm mean squared brightness temperature fluctuations at $k=1 \,{\rm Mpc}^{-1}$.

==> preamble.tex <==
\makeatletter
\newcommand{\ifmnras}[2]{\@ifclassloaded{mnras}{#1}{#2}}
\makeatother
\makeatletter
\newcommand{\ifpasa}[2]{\@ifclassloaded{cup-journal}{#1}{#2}}
\makeatother
% % Font and Input
\ifpasa{\usepackage[nopatch]{microtype}}{\usepackage{microtype}}
\usepackage[T1]{fontenc}
\ifpasa{}{\usepackage[utf8]{inputenc}}
\usepackage{multicol}
\ifpasa{}{\usepackage{newtxtext,newtxmath}}
\usepackage{ae,aecompl}
\usepackage{fix-cm}

% % Linguistic
\usepackage[english]{babel}
\usepackage{csquotes}

% % Layout
\usepackage[svgnames]{xcolor}
\definecolor{equationCol}{HTML}{D95F02}
\definecolor{sectionCol}{HTML}{7570B3}
\definecolor{citeCol}{HTML}{1B9E77}

% \ifmnras{\usepackage{hyperref}}{\usepackage[colorlinks=true, linkcolor=sectionCol, citecolor=citeCol]{hyperref}}
\ifmnras{\usepackage{hyperref}}{\usepackage[colorlinks=true,linkcolor=blue, citecolor=blue, allcolors=blue]{hyperref}}


\ifpasa{}{\ifmnras{}{\usepackage[a4paper, width=200mm, top=25mm, bottom=25mm]{geometry}}}

\usepackage{fancyhdr}
\pagestyle{fancy}
\ifpasa{}{\usepackage{titlesec}}
\ifpasa{}{\usepackage{cleveref}}

\ifpasa{}{\crefformat{footnote}{#2\footnotemark[#1]#3}}

% % Math
\usepackage{mathtools}
\usepackage{amsmath}
\ifmnras{}{\usepackage{amssymb}}
\usepackage{nicefrac}
\ifpasa{}{\usepackage{breqn}}
\usepackage{gensymb}

% % Tables
\usepackage{array}
\usepackage{booktabs}
\usepackage{arydshln}
\renewcommand{\arraystretch}{1.2}

% % Graphics
\usepackage{subcaption}
% \usepackage{subfigure}
\usepackage{graphicx}
\usepackage{float}

% % Science
\usepackage{siunitx}

% % Bibliography
\ifpasa{}{\ifmnras{}{\usepackage[natbibapa, nodoi]{apacite}}}

\ifpasa{}{\ifmnras{}{\usepackage{natbib}}}

\usepackage{booktabs}
\renewcommand{\arraystretch}{1.2}

% The Astrophysical Journal -> ApJ
\ifpasa{}{\ifmnras{}{\newcommand{\apj}{ApJ}}}

% The Astronomical Journal -> AJ
\ifpasa{}{\ifmnras{}{\newcommand{\aj}{AJ}}}

% The Astrophysical Journal Letters -> ApJL
\ifpasa{}{\ifmnras{}{\newcommand{\apjl}{ApJL}}}

% Monthly Notices of the Royal Astronomical Society -> MNRAS
\ifpasa{}{\ifmnras{}{\newcommand{\mnras}{MNRAS}}}

% Publications of the Astronomical Society of the Pacific -> PASP
\ifpasa{}{\ifmnras{}{\newcommand{\pasp}{PASP}}}

% Nature -> Nature
\ifpasa{}{\ifmnras{}{\newcommand{\nat}{Nature}}}

%
\ifpasa{}{\ifmnras{}{\newcommand{\aap}{AAP}}}

%
\ifpasa{}{\ifmnras{}{\newcommand{\prl}{Phys. Rev. Lett.}}}

% % User Defined Functions

% % Redefine eqref
\newcommand*{\SavedEqref}{}
\let\SavedEqref\eqref
\renewcommand*{\eqref}[1]{%
    \begingroup
        \hyperseup{
            linkcolor=equationCol,
            linkbordercolor=equationCol,
        }%
        \SavedEqref{#1}%
    \endgroup
}

% Column Vector
\newcommand*\cvec[1]{\begin{bmatrix}#1\end{bmatrix}}

% Line Break
\newcommand*\lbreak{\\[\baselineskip]}

%%%%%%%%%%%%% alias %%%%%%%%%%%%%
\defcitealias{Chatterjee2022}{Paper~I}
